Cost-Sensitive Multi-Fidelity Bayesian Optimization with Transfer of Learning Curve Extrapolation

In this paper, we address the problem of cost-sensitive multi-fidelity Bayesian Optimization (BO) for efficient hyperparameter optimization (HPO). Specifically, we assume a scenario where users want to early-stop the BO when the performance improvement is not satisfactory with respect to the required computational cost. Motivated by this scenario, we introduce utility, which is a function predefined by each user and describes the trade-off between cost and performance of BO. This utility function, combined with our novel acquisition function and stopping criterion, allows us to dynamically choose for each BO step the best configuration that we expect to maximally improve the utility in future, and also automatically stop the BO around the maximum utility. Further, we improve the sample efficiency of existing learning curve (LC) extrapolation methods with transfer learning, while successfully capturing the correlations between different configurations to develop a sensible surrogate function for multi-fidelity BO. We validate our algorithm on various LC datasets and found it outperform all the previous multi-fidelity BO and transfer-BO baselines we consider, achieving significantly better trade-off between cost and performance of BO.

==> captions/introduction_caption.tex <==
\begin{figure}[t]
\vspace{-0.2in}
\begin{subfigure}[c]{0.345\textwidth}
\centering
    \includegraphics[height=3.75cm]{figures/csbo.pdf}
    \vspace{-0.07in}
\subcaption{}
\label{fig:csbo}
\end{subfigure}
\begin{subfigure}[c]{0.345\textwidth}
\centering
    \includegraphics[height=3.75cm]{figures/utility.pdf}
    \vspace{-0.07in}
\subcaption{}
\label{fig:utility}
\end{subfigure}
\begin{subfigure}[c]{0.3\textwidth}
\centering
    \includegraphics[height=3.75cm]{figures/beta.pdf}
    \vspace{-0.07in}
\subcaption{}
\label{fig:beta}
\end{subfigure}
\vspace{-0.13in}
\caption{\small \textbf{(a)} An illustration of a utility function shown in the dotted black lines. The red curve shows a BO trajectory from which we determine the maximum utility ($\approx$ 0.7) and when to stop ($b^*$). \textbf{(b)} An illustration of deciding which configuration to select at each BO step. Note that the y-axis is utility. Starting from the current BO step $b$, we extrapolate the LCs with the three configurations $x_1,x_2,x_3$ (shown in the solid curves with colors and the shaded area), and then select $x_3$ which achieves at $b_3$ the maximum expected improvement (EI) of utility over the previous utility $U_\text{prev}$. \textbf{(c)} Eq.~\eqref{eq:threshold} with $\gamma=\log_2 5$ and the various values for $\beta$.}
\label{fig:concepts}
\vspace{-0.2in}
\end{figure}

==> captions/lcbench.tex <==
\begin{table}[t!]
\small
\centering
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\small
%\resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccccccccccccc|c}
    \midrule[0.8pt]
    %& \multicolumn{15}{c}{$(b_{min}, \alpha) = (20, 5e^{5})$} \\ 
    %\midrule[0.8pt]
    Method & $\mathcal{D}_1$ & $\mathcal{D}_2$ & $\mathcal{D}_3$ & $\mathcal{D}_4$ & $\mathcal{D}_5$ & $\mathcal{D}_6$ & $\mathcal{D}_7$ & $\mathcal{D}_8$ & $\mathcal{D}_9$ & $\mathcal{D}_{10}$ & $\mathcal{D}_{11}$ & $\mathcal{D}_{12}$ & $\mathcal{D}_{13}$ & $\mathcal{D}_{14}$ & $\mathcal{D}_{15}$ & Avg. \\    
    \midrule[0.8pt]
    Random & 0.99 & 1.05 & 1.18 & 0.72 & 1.55 & 0.99 & 1.01 & 1.45 & 1.94 & 1.17 & 0.69 & 0.62 & 1.16 & 0.51 & 0.79 & 1.05\\
    HyperBand & 1.07 & 1.06 & 1.26 & 0.71 & 1.35 & 0.85 & 1.09 & 1.52 & 2.09 & 1.07 & 0.43 & 0.69 & 1.12 & 0.67 & 0.80 & 1.05 \\
    BOHB & 1.22 & 1.17 & \bf1.71 & 0.74 & 1.41 & 1.33 & \bf1.64 & 1.57 & 2.00 & 1.36 & 1.09 & 0.74 & 1.38 & 0.93 & 0.87 & 1.28 \\
    DEHB & 1.06 & 1.06 & 1.43 & 0.74 & 1.40 & 1.21 & 1.37 & \bf1.66 & \bf2.22 & 1.05 & 1.00 & 0.58 & 1.35 & 0.78 & 0.97 & 1.19 \\
    ASHA & 1.07 & 1.06 & 1.26 & 0.71 & 1.35 & 0.85 & 1.09 & 1.52 & 2.09 & 1.07 & 0.43 & 0.69 & 1.12 & 0.67 & 0.80 & 1.05 \\
    DyHPO & 1.14 & 1.08 & 1.69 & 0.69 & \bf1.64 & 1.32 & \bf1.64 & 1.52 & 1.87 & 1.19 & 1.15 & 0.61 & 1.24 & 1.04 & 0.97 & 1.25  \\
    TDyHPO & 1.29 & 1.08 & 1.55 & 0.85 & 1.46 & 1.06 & 1.46 & 1.45 & 2.02 & 1.28 & 1.07 & 0.60 & 1.02 & 0.94 & 0.84 & 1.20\\
    \midrule[0.8pt]  
    Ours & \bf2.44 & \bf1.73 & 1.57 & \bf1.68 & 1.39 & \bf1.83 & \bf1.64 & 1.62 & \bf2.22 & \bf1.96 & \bf2.52 & \bf0.76 & \bf1.49 & \bf1.17 & \bf1.33 & \bf 1.69 \\
    \midrule[0.8pt]  
\end{tabular}
%}
\caption{\small The results of \textbf{architecture generalization}. ConvNet4 is utilized for condensing TinyImageNet into 2,000 synthetic examples. Models with different architectures are pretrained on the condensed dataset and finetuned on target datasets. We report the average and standard deviation over three runs. }
\label{tab:architecture}
\vspace{0.2in}
\end{table}

==> captions/mixup.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-0.2in}
\begin{subfigure}[c]{0.24\textwidth}
\centering
    \includegraphics[height=3cm]{figures/meta_mixup.pdf}
    \vspace{-0.1in}
\subcaption{Meta-Mixup}
\label{fig:meta_mixup}
\end{subfigure}
\begin{subfigure}[c]{0.24\textwidth}
\centering
    \includegraphics[height=3cm]{figures/hparam_mixup.pdf}
    \vspace{-0.1in}
\subcaption{Hparam-Mixup}
\label{fig:hparam_mixup}
\end{subfigure}
\vspace{-0.2in}
\end{wrapfigure}

==> captions/overfit.tex <==
\begin{figure}[H]
\vspace{-0.1in}
\begin{subfigure}[c]{0.245\textwidth}
\centering
    \includegraphics[height=3.4cm]{figures/overfit_lcbench.pdf}    
\subcaption{}
\label{fig:overfit_lcbench}
\end{subfigure}
\begin{subfigure}[c]{0.245\textwidth}
\centering
    \includegraphics[height=3.4cm]{figures/overfit_taskset.pdf}    
\subcaption{}
\label{fig:overfit_taskset}
\end{subfigure}
\begin{subfigure}[c]{0.245\textwidth}
\centering
    \includegraphics[height=3.4cm]{figures/overfit_pd1.pdf}   
\subcaption{}
\label{fig:overfit_pd1}
\end{subfigure}
\begin{subfigure}[c]{0.245\textwidth}
\centering
    \includegraphics[height=3.4cm]{figures/pd1_mixup_ablation.pdf}    
\subcaption{}
\label{fig:overfit_pd1_hpo}
\end{subfigure}
\vspace{-0.1in}
\caption{\small \textbf{(a, b, c)} Visualization of test loss on unseen LC datasets in LCBench, TaskSet, and PD1, respectievly. \textbf{(d)} Conventional multi-fidelity BO ($\alpha=0$) results on PD1. }
\vspace{-0.1in}
\end{figure}

==> captions/utility.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-0.2in}
\centering
    \includegraphics[height=4cm]{figures/utility.pdf}    
    \vspace{-0.1in}
\caption{\small A graphical illustration on our proposed utility space. Here y-axis is the cumulative performance, not the utility as illustrated in Figure~\ref{fig:introduction_b} and \ref{fig:introduction_c}. Blue lines are predicted learning curves, where sky blue arrows denote the projection. }
\label{fig:utility}
\vspace{-0.2in}
\end{wrapfigure}

==> sections/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In the experimental section, we provided numerous supporting evidences for the claims made in the paper.

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the \textbf{Limitations} paragraph in \S\ref{sec:conclusion}.

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not include any theoretical claims.

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide experimental details including datasets, training details, and baseline implementation  throughout \S\ref{sec:data} and \ref{sec:additional_setups}.

\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We use public benchmark datasets and upload anonymous code in the supplemental materials.


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We not only provide experimental setups in main paper but also detail the setups in depth throughout \S\ref{sec:data} and \ref{sec:additional_setups}.

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide mean and standard deviation over 5 runs for all our experiments.

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide the detailed information in the Appendix.
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: We carefully reviewed the NeurIPS Code of Ethics.


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The topic of our paper is about improving the efficiency of hyperparameter optimization, which is irrelevant to societal impacts.
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{}
    \item[] Justification: Our paper is not relevant to such issues and risks.

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}.
    \item[] Justification: Yes, we properly put citations and URLs for them throughout the paper.

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification: Our paper does not release any new assets.

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: Our paper does not involve any crowdsourcing nor research with human subjects.

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}.
    \item[] Justification: Our paper does not involve any crowdsourcing nor research with human subjects.

\end{enumerate}

